Differential biases, $c$-differential uniformity, and their relation to differential attacks

Differential cryptanalysis famously uses statistical biases in the propagation of differences in a block cipher to attack the cipher. In this paper, we investigate the existence of more general statistical biases in the differences. To this end, we discuss the $c$-differential uniformity of S-boxes, which is a concept that was recently introduced in Ellingsen et. al. to measure certain statistical biases that could potentially be used in attacks similar to differential attacks. Firstly, we prove that a large class of potential candidates for S-boxes necessarily has large $c$-differential uniformity for all but at most $B$ choices of $c$, where $B$ is a constant independent of the size of the finite field $q$. This result implies that for a large class of functions, certain statistical differential biases are inevitable. In a second part, we discuss the practical possibility of designing a differential attack based on weaknesses of S-boxes related to their $c$-differential uniformity.

==> avanzi-tikz-defs.tex <==
\usepackage{tikz}

\usetikzlibrary{arrows}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{chains}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{fit}
\usetikzlibrary{intersections}
\usetikzlibrary{matrix}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{trees}

\tikzset{>=latex}

\tikzset{
  register/.style={
    rectangle, 
    draw=black, thick,
    minimum height=1.66em, 
    text centered,
  },
  block/.style={
    rectangle, 
    rounded corners, 
    draw=black, thick,
    minimum height=1.66em, 
    text centered,
  },
  thickrect/.style={
    rectangle, 
    draw=black, thick,
    minimum height=1.66em, 
    text centered,
  },
  wideblock/.style={
    block, 
    minimum width=30mm,
  },
  midblock/.style={
    block, 
    minimum width=15mm,
  },
  midsquaredblock/.style={
    block, 
    rounded corners=false,
    minimum width=15mm,
  },
  smallfunction/.style={
    rectangle, 
    rounded corners, 
    draw=black, thick,
    minimum height=1.66em, 
    text centered,
  },
  function/.style={
    smallfunction, 
    minimum width=0.8cm,
  },
  widefunction/.style={
    smallfunction,
    minimum width=30mm,
  },
  cross line/.style={preaction={draw=white, -, shorten >=1pt, shorten <=1pt, line width=3.33pt}},
  arrow/.style = {->,black,semithick},
  doublearrow/.style = {<->,black,semithick},
  worra/.style = {<-,black,semithick}, %% reverse arrow
  connect/.style = {-,semithick},
  decoration={brace},
}

\def\branch#1{\fill #1 circle [radius=1.5pt];}

\tikzset{XOR/.style=
          {draw,circle,thick,fill=white,scale=1.1,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            (\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
            (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)}
          },
         AND/.style=
          {draw,circle,thick,fill=white,scale=1.1,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            (\tikzlastnode.north) edge[thick] (\tikzlastnode.south east)
            (\tikzlastnode.north) edge[thick] (\tikzlastnode.south west)}
          },
         OR/.style=
          {draw,circle,thick,fill=white,scale=1.1,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            (\tikzlastnode.south) edge[thick] (\tikzlastnode.north east)
            (\tikzlastnode.south) edge[thick] (\tikzlastnode.north west)}
          },
         NOT/.style=
          {draw,circle,thick,fill=white,scale=1.1,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            ($(\tikzlastnode.west)+(1.5pt,-0.625pt)$) edge[thick,out=60,in=240,looseness=2] ($(\tikzlastnode.east)-(1.5pt,-0.625pt)$)
            }
          },
         PLUS/.style=
          {draw,rectangle,thick,fill=white,scale=1.5,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            (\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
            (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)}
          },
         MINUS/.style=
          {draw,rectangle,thick,fill=white,scale=1.5,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)}
          },
         TIMES/.style=
          {draw,circle,thick,fill=white,scale=1.1,append after command={
            [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
            (\tikzlastnode.south west) edge[thick] (\tikzlastnode.north east)
            (\tikzlastnode.south east) edge[thick] (\tikzlastnode.north west)}
          },
         MULT/.style=
          {draw,circle,thick,fill=white,scale=1.1, append after command={
             node[fill,circle,thick,inner sep=0.3mm] at (\tikzlastnode) {} }
          },
         COMP/.style=
          {draw,circle,thick,fill=white,scale=1.1, append after command={
             node[draw,circle,thick,inner sep=0.6mm] at (\tikzlastnode) {} }
          },
         COMPAST/.style=
          {draw,circle,thick,fill=white,scale=1.1, append after command={
             node[] at ($(\tikzlastnode)+(0.1pt,-0.3pt)$) (tmp) {\scalebox{1.333}{$\ast$}}  }
          },
         branch/.style=
           {fill,shape=circle,minimum size=3pt,inner sep=0pt},
         bit/.style=
           {fill,shape=rectangle,minimum size=0.5mm,inner sep=0pt},
}




==> tikzlibrarycrypto.symbols.code.tex <==
\usetikzlibrary{arrows}			%% Include regular arrows
%\usepgflibrary{arrows.new}		%% Include custom arrows
\usetikzlibrary{shadows.blur}	%% Include the package to add shadows

%%
%% XOR in TIKZ
%%
\tikzset{XOR/.style={thick,
					draw,
					circle,
					append after command={
					        [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
					        (\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
					        (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)
        				},
    				},
}

%%
%% ADD in TIKZ
%%
\tikzset{ADD/.style={thick,
					draw,
					rectangle,
					append after command={
					        [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
					        (\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
					        (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)
				        },
				    },
}

%%
%% MOD ADD in TIKZ
%%
\tikzset{MODADD/.style={thick,
						draw,
						rectangle,
						append after command={
								[shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
								(\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
								(\tikzlastnode.east) edge[thick] (\tikzlastnode.west)
							},
						},
}

%%% Shadows
\tikzset{
		%% XOR node
		shadows/.is choice,
		shadows/yes/.style={
			XOR/.append style={fill=white,blur shadow={shadow blur steps=5}},
			ADD/.append style={blur shadow={shadow blur steps=5}},
			MODADD/.append style={fill=white,blur shadow={shadow blur steps=5}}
		},
		shadows/no/.style={
		},
		%% Default: no shadows
		shadows = no,
}


%%%%%%%%%%%%%%%%%%%%%% AUTHENTICATED ENCRYPTION %%%%%%%%%%%%%%%%%%%%

%%
%% AE: Message block
%%
\tikzset{AE_msg/.style={
		rectangle,
		thick,
		draw,
		fill=blue!20,
		text width=1cm,
		minimum height=0.5cm,
		text centered,
		anchor=north,
	}
}

%%
%% AE: Ciphertext block
%%
\tikzset{AE_ctx/.style={
		rectangle,
		thick,
		draw,
		fill=green!20,
		text width=1cm, 
		minimum height=0.5cm,
		text centered,
		anchor=north,
	}
}

%%
%% AE: Tag block
%%
\tikzset{AE_tag/.style={
		rectangle,
		thick,
		draw,
		fill=red!20,
		text width=1cm, 
		minimum height=0.5cm,
		text centered,
		anchor=north,
	}
}

%%
%% AE: Block cipher call
%%
\tikzset{AE_E/.style={
		rectangle,
		thick,
		draw,
		fill=yellow!20,
		text width=1cm, 
		minimum height=1cm,
		text centered,
		anchor=north,
	}	
}

%%%%%%%%%%%%%%%%%%%%%%%%%% Custom lines or arrows %%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzset{edge/.style={
						-latex new, 
						arrow head=8pt, 
						thick
					},
}

\tikzset{line/.style={
						thick,
						draw, 
						-latex',
						shorten <=1bp,
						shorten >=1bp,
					}
}

\tikzset{doublearrow/.style={
								thick,
								draw, 
								latex-latex,
								shorten <=1bp,
								shorten >=1bp
							}
}

\tikzset{edgee/.style={
						latex new-latex new, 
						arrow head=8pt, 
						thick,
						}
}

\tikzset{Redge/.style={
						latex new-, 
						arrow head=8pt, 
						thick,
						}
}


